RFCLLM: Evaluating LLMs' Reasoning Ability of Network Protocol State Machines

Mapping textual specifications into formal representations is essential for ensuring the correctness of protocol designs and implementations. LLM-generated mappings, used for networking security or testing, are assumed to capture a perfect understanding of the specification, which may not hold in practice. The goal of this paper is to assess the extent to which LLMs can interpret the specification correctly. We examine the degree to which an LLM's implicit representation of a finite-state transition system-defined via natural language descriptions-aligns with a manually generated ground-truth model. We designed 4 tasks and 1482 task queries for 16 protocols. We evaluated different judge biases, observed the inherent difficulty gaps between tasks, looked into the effect of 4 context types, and the influence of protocol characteristics. Our work contributes to a step toward verifying whether LLMs can really be trusted in FSM (Finite State Machine) reasoning of protocol specifications.

==> eval-dsr1-qwen-32b.tex <==

\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 1 results (deepseek-r1-distilled-qwen-32B). \anqi{have not yet run 7b judge}}
\begin{tabular}{p{2.2cm}|p{3.5cm}| p{1.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $s'$ \newline (judges: 0.6-sim, llama3.3-70b) &  \#Correct $A'$ \newline (judges: 0.6-sim, llama3.3-70b) & \#Correct both \newline (judges: 0.6-sim, llama3.3-70b) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 15
    & 15, 15 \newline 7, 7 \newline 8, 8 
    & 13, 13 \newline 4, 9 \newline 8, 10
    & 13,  13 \newline 2, 4 \newline 5, 7  \\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 15
    & 15, 15 \newline 8, 8 \newline 9, 9
    & 15, 15\newline 0, 1  \newline 0, 1
    & 15, 15 \newline 0, 0\newline 0, 1  \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 27
   & 26, 27  \newline 24, 22  \newline 18, 17
    & 26, 26\newline 12, 11 \newline 3, 6
    & 26, 26 \newline 12, 11 \newline 3, 5 \\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 21
   & 21, 21 \newline 16, 14 \newline 16, 15
    & 21, 21 \newline 6, 10\newline 6, 10
    & 21, 21 \newline 5, 8\newline 4, 7\\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 34
   & 34, 34\newline 16, 20 \newline 15, 19
    & 34, 34 \newline 4, 10 \newline 3, 14
    & 34, 34 \newline 3, 8 \newline 3, 10\\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 21
    & 19, 19 \newline 18, 19 \newline 11, 13
    & 19, 19 \newline 8, 8 \newline 3, 4
    & 19, 19 \newline 8, 8 \newline 3, 3 \\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 15, 19\newline 12, 11 \newline 14, 13
    & 15, 15 \newline 4, 3 \newline 4, 5
    & 15, 15\newline 2, 2 \newline 3, 3 \\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 24
   & 24, 24\newline 23, 23  \newline 16, 16 
    & 22, 21 \newline 8, 9\newline 0, 0
    & 22, 21 \newline 8, 9\newline 0, 0  \\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 23
    & 23, 23 \newline 18, 18 \newline 19, 19 
    & 23, 18  \newline 5, 9\newline 4, 10
    & 23, 18 \newline 3, 7 \newline 3, 9\\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 18
    & 18, 18 \newline 13, 13  \newline 9, 9
    & 18, 18 \newline 1, 7\newline 2, 9 
    & 18, 18 \newline 1, 5\newline 1, 5\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 9
    & 9, 9 \newline 8, 8 \newline 9, 9
    & 9, 9 \newline 1, 2 \newline 1, 1
    & 9, 9 \newline 1, 1\newline 1, 1 \\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 14
    & 14, 14 \newline 3, 5   \newline 3, 4
    & 14, 14  \newline 4, 5 \newline 4, 5 
    & 14, 14 \newline 2, 3 \newline 1, 4 \\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 20
    & 20, 20  \newline 19, 19  \newline 8, 12
    & 20, 20 \newline 5, 6 \newline 5, 4
    & 20, 20 \newline 5, 6 \newline 3, 2 \\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 33
    & 25, 25 \newline 23, 23  \newline 9, 9 
    & 20, 20  \newline 0, 0\newline 1, 2
    & 20, 20 \newline 0, 0 \newline 0, 2 \\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 24
   & 18, 17\newline 8, 10 \newline 1, 4
    & 19, 17 \newline 2, 11\newline 1, 3
    & 18, 17 \newline 0, 5 \newline 0, 0  \\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
   &  17, 17\newline 10, 10 \newline 9, 9
    & 17, 17 \newline 4, 4\newline 2, 4
    & 17, 17 \newline 2, 3 \newline 1, 3 \\

\bottomrule
\end{tabular}
\label{tab:task1-32b}
\end{table*}

\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 2 results (deepseek-r1-distilled-qwen-32B). \anqi{have not yet run 7b judge}}
\begin{tabular}{p{2.5cm}|p{4cm}|p{2.5cm}|p{4cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $C'$ \newline 
(judges: 0.6-sim, llama3.3-70b) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 15
    & 13, 13\newline 1, 6,  \newline 0, 3, \\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 12
    & 11, 11\newline 1, 4 \newline 1, 4\\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted\newline No context
    & 19
    & 16, 16\newline 4, 4\newline 2, 2\\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 17\newline 1, 7  \newline 1, 3 \\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 22
    & 20, 19\newline 0, 0  \newline 0, 3 \\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 20
    & 19, 19 \newline 4, 4 \newline 0, 1\\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 16
    & 15, 14 \newline 2, 3 \newline 2, 4\\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 13, 13\newline 2, 2 \newline 1, 0 \\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted\newline No context 
    & 17
    & 17, 17\newline 5, 5  \newline 1, 2 \\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 6
    & 5, 5 \newline 1, 2 \newline 0, 1\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 9
    & 6, 7 \newline 4, 5\newline 4, 6 \\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 12
    & 12, 12 \newline 0,  0 \newline 0, 2 \\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 11
    & 10, 10 \newline 1, 3 \newline 1, 1\\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 8
    & 2, 2\newline 0, 0 \newline 0, 0\\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 18, 18 \newline 1, 0 \newline 2, 1\\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    &17, 17\newline 0, 0 \newline 1, 0\\

\bottomrule
\end{tabular}
\label{tab:task2-32b}
\end{table*}

\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 3 results (deepseek-r1-distilled-qwen-32B). \anqi{have not yet run 7b judge}}
\begin{tabular}{p{2.5cm}|p{4cm}|p{2.5cm}|p{4cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $S_i$ \newline 
(judges: 0.6-sim, llama3.3-70b ) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 13
    & 10, 9  \newline 3, 2   \newline  4, 2\\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 11
    & 4, 4 \newline 2, 2  \newline 1, 1 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted\newline No context
    & 14
    & 13, 9 \newline 8, 4 \newline 4, 3 \\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 12, 7 \newline 6, 1 \newline 6, 2\\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 28
    & 19, 15 \newline 9, 9 \newline 4, 3 \\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 18, 15 \newline 8, 8\newline 5, 5\\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 14
    & 7, 4 \newline 2, 1 \newline 2, 1\\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 15, 12 \newline 9, 8 \newline 4, 3 \\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 7, 7 \newline 8, 8 \newline 8, 8 \\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 15, 14 \newline 9, 9\newline 8, 8\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 7
    & 6, 2\newline  3, 2\newline 4, 4\\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 12
    & 11, 4 \newline 0, 0\newline 0, 0 \\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted  \newline No context
    & 15
    & 7, 7\newline 6, 5 \newline 2, 3 \\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 22
    & 10, 10 \newline 4, 4 \newline 3, 3\\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 14, 12\newline 0, 3 \newline 0, 0 \\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 12, 11 \newline 0, 0 \newline 0, 0 \\

\bottomrule
\end{tabular}
\label{tab:task3-32b}
\end{table*}

==> eval-gemini3flashpreview.tex <==

\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 1 results (gemini-3-flash-preview).}
\begin{tabular}{p{2.2cm}|p{3.5cm}| p{1.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $s'$ \newline (judges: 0.6-sim, llama3.3-70b) &  \#Correct $A'$ \newline (judges: 0.6-sim, llama3.3-70b) & \#Correct both \newline (judges: 0.6-sim, llama3.3-70b) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 15
    & 15, 15 \newline 14, 14  \newline 14, 14 \newline 12, 13
    & 15, 13 \newline 5, 10 \newline 11, 10 \newline 11, 12 
    & 13, 13 \newline 4, 9 \newline 10, 9 \newline 9, 11 \\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 15
     & 15, 15 \newline 8, 8 \newline 8, 8 \newline 9, 10
    & 15, 15 \newline 0, 1 \newline 0, 1 \newline 0, 0
    & 15, 15 \newline 0, 1 \newline 0, 1 \newline 0, 0 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 27
     & 27, 27 \newline 25, 24 \newline 25, 25 \newline 24, 23 
    & 26, 27 \newline 17, 10 \newline 3, 8 \newline 7, 10 
    & 26, 27 \newline 15, 9 \newline 3, 8 \newline 7, 10 \\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted  \newline No context
    & 21
   & 21, 21 \newline 19, 18 \newline 18, 17 \newline 16, 12
    & 21, 21 \newline 8, 12 \newline 7, 8 \newline 3, 6
    & 21, 21 \newline 7, 10 \newline 6, 7 \newline 3, 5\\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 34
   & 34, 34\newline 19, 20 \newline 12, 14 \newline 9, 9
    & 34, 33 \newline 3, 10 \newline 3, 12 \newline 7, 10
    & 34, 33 \newline 2, 4 \newline 3, 4 \newline 0, 0\\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 21
    & 20, 20 \newline 16, 17 \newline 13, 16 \newline 3, 4
    & 20, 20 \newline 12, 10 \newline 6, 6 \newline 1, 4 
    & 20, 20 \newline 10, 9 \newline 6, 6 \newline 0, 0\\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 19, 19\newline 12, 11 \newline 12, 12 \newline 14, 13
    & 16, 17 \newline 9, 8 \newline 4, 6 \newline 4, 6
    & 16, 17\newline 5, 4 \newline 2, 4 \newline 4, 4 \\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 24
   & 24, 24\newline 24, 17  \newline 18, 19 \newline 15, 15
    & 24, 23 \newline 21, 10\newline 0, 0 \newline 0, 0
    & 24, 23 \newline 21, 9\newline 0, 0 \newline 0, 0\\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 23
     & 23, 23 \newline 21, 21 \newline 18, 18 \newline 18, 18
    & 23, 18 \newline 0, 5 \newline 0, 2 \newline 2, 3
    & 23, 18 \newline 0, 5 \newline 0, 2 \newline 2, 3\\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 18
    & 18, 18 \newline 12, 13  \newline 12, 12 \newline 13, 13
    & 17, 17 \newline 2, 8 \newline 3, 5 \newline 2, 7 
    & 17, 17 \newline 0, 6\newline 1, 3 \newline 2, 5\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 9
    & 9, 9 \newline 9, 9 \newline 9, 9 \newline 6, 6
    & 9, 9 \newline 3, 3 \newline 3, 3 \newline 2, 2
    & 9, 9 \newline 3, 3\newline 3, 3 \newline 2, 2  \\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 14
    & 14, 14 \newline 7, 7   \newline 6, 4 \newline 0, 6
    & 14, 14  \newline 3, 7 \newline 6, 7 \newline 1, 5
    & 14, 14 \newline 2, 5 \newline 4, 4 \newline 0, 1\\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 20
    & 20, 20  \newline 19, 19  \newline 15, 15 \newline 13, 15
    & 20, 20 \newline 8, 14 \newline 4, 6 \newline 2, 2
    & 20, 20 \newline 8, 14 \newline 3, 4 \newline 2, 2 \\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 33
    & 28, 28 \newline 21, 21  \newline 8, 8 \newline 11, 9  
    & 16, 10  \newline 3, 1 \newline 0, 2 \newline 0, 1
    & 16, 10 \newline 2, 1 \newline 0, 1 \newline 0, 1 \\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 24
   & 20, 18 \newline 11, 16 \newline 0, 3 \newline 6, 6
    & 24, 18 \newline 5, 12\newline 0, 11 \newline 0, 11
    & 20, 18 \newline 0, 11 \newline 0, 3 \newline 0, 2 \\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 17 \newline 11, 10  \newline 10, 12 \newline 10, 12 
    & 17, 17 \newline 3, 5 \newline 3, 4 \newline 1, 4
    & 17, 17 \newline 2, 3\newline 3, 3 \newline 1, 4 \\

\bottomrule
\end{tabular}
\label{tab:task1-gemini3fp}
\end{table*}



\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 2 results (gemini-3-flash-preview).}
\begin{tabular}{p{2.5cm}|p{4cm}|p{2.5cm}|p{4cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $C'$ \newline 
(judges: 0.6-sim, llama3.3-70b) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 15
     &14, 14 \newline 3, 6 \newline 1, 3 \newline 3, 5\\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 12
     &12, 12\newline 4, 6 \newline 5, 8 \newline 2, 1 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 19
     &15, 15 \newline 4, 6 \newline 4, 5 \newline 0, 2 \\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 17\newline 1, 7  \newline 1, 7 \newline 0, 1 \\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 22
    & 21, 21\newline 0, 4  \newline 0, 0 \newline 0, 0 \\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 20
    & 17, 17 \newline 7, 4 \newline 2, 3 \newline 1, 1 \\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 16
    & 16, 15 \newline 6, 5 \newline 5, 5 \newline 0, 1 \\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 12, 12\newline 4, 5 \newline 0, 0 \newline 0, 1 \\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 16, 16 \newline 2, 3 \newline 2, 2 \newline 3, 5 \\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 6
    & 6, 6 \newline 2, 3 \newline 2, 3 \newline 1, 1 \\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 9
    & 6, 5 \newline 4, 2\newline 4, 3 \newline 3, 4 \\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 12
    & 12, 12 \newline 1,  1 \newline 0, 0 \newline 0, 0 \\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 11
    & 9, 9 \newline 1, 3 \newline 0, 4 \newline 0, 0\\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 8
    & 3, 3\newline 0, 1 \newline 0, 0 \newline 0, 0 \\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 18, 18 \newline 2, 0 \newline 3, 2 \newline 1, 2 \\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    &16, 17 \newline 0, 2 \newline 1, 1 \newline 0, 0\\

\bottomrule
\end{tabular}
\label{tab:task2-gemini3fp}
\end{table*}



\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 3 results (gemini-3-flash-preview). }
\begin{tabular}{p{2.5cm}|p{4cm}|p{2.5cm}|p{4cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $S_i$ \newline 
(judges: 0.6-sim, llama3.3-70b ) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 13
     & 10, 8 \newline 4, 2 \newline 5, 3 \newline 5, 4 \\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 11
    &7, 7\newline 2, 2 \newline 2, 2 \newline 0, 0 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 14
     & 14, 9\newline 10, 6 \newline 10, 4 \newline 10, 5\\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 14, 8 \newline 7, 1 \newline 6, 2 \newline 3, 0\\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 28
    & 17, 15 \newline 0, 0 \newline 0, 0 \newline 0, 1 \\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 19, 16 \newline 11, 8\newline 6, 7 \newline 0, 0\\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 14
    & 7, 4 \newline 2, 1 \newline 2, 2 \newline 2, 1\\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 16, 13 \newline 5, 5 \newline 8, 7 \newline 2, 2\\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 6, 6 \newline 4, 4 \newline 9, 9 \newline 8, 8\\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 14 \newline 12, 13\newline 12, 13 \newline 7, 5\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 7
    & 7, 3\newline  4, 5\newline 4, 4 \newline 1, 1\\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 12
    & 12, 4 \newline 1, 1\newline 0, 0 \newline 1, 1\\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 10, 10\newline 8, 8\newline 2, 2 \newline 1, 2\\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 22
    & 11, 11 \newline 4, 4 \newline 6, 6 \newline 2, 2\\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 15, 13\newline 1, 2 \newline 1, 1 \newline 0, 0\\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 13, 12 \newline 1, 0 \newline 2, 0 \newline 3, 1\\

\bottomrule
\end{tabular}
\label{tab:task3-gemini3fp}
\end{table*}

==> eval-gpt-4o-mini.tex <==

\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}

\caption{Task 1 results (gpt-4o-mini). \anqi{the numbers for gpt4o and gemini3flashrpeview have not been written }}
\begin{tabular}{p{2.2cm}|p{3.5cm}| p{1.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $s'$ \newline (judges: 0.6-sim, llama3.3-70b) &  \#Correct $A'$ \newline (judges: 0.6-sim, llama3.3-70b) & \#Correct both \newline (judges: 0.6-sim, llama3.3-70b) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 15
    & 15, 15 \newline 14, 14  \newline 14, 14 \newline 12, 13
    & 15, 13 \newline 5, 10 \newline 11, 10 \newline 11, 12 
    & 13, 13 \newline 4, 9 \newline 10, 9 \newline 9, 11 \\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 15
     & 15, 15 \newline 8, 8 \newline 8, 8 \newline 9, 10
    & 15, 15 \newline 0, 1 \newline 0, 1 \newline 0, 0
    & 15, 15 \newline 0, 1 \newline 0, 1 \newline 0, 0 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 27
     & 27, 27 \newline 25, 24 \newline 25, 25 \newline 24, 23 
    & 26, 27 \newline 17, 10 \newline 3, 8 \newline 7, 10 
    & 26, 27 \newline 15, 9 \newline 3, 8 \newline 7, 10 \\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted  \newline No context
    & 21
   & 21, 21 \newline 19, 18 \newline 18, 17 \newline 16, 12
    & 21, 21 \newline 8, 12 \newline 7, 8 \newline 3, 6
    & 21, 21 \newline 7, 10 \newline 6, 7 \newline 3, 5\\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 34
   & 34, 34\newline 19, 20 \newline 12, 14 \newline 9, 9
    & 34, 33 \newline 3, 10 \newline 3, 12 \newline 7, 10
    & 34, 33 \newline 2, 4 \newline 3, 4 \newline 0, 0\\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 21
    & 20, 20 \newline 16, 17 \newline 13, 16 \newline 3, 4
    & 20, 20 \newline 12, 10 \newline 6, 6 \newline 1, 4 
    & 20, 20 \newline 10, 9 \newline 6, 6 \newline 0, 0\\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 19, 19\newline 12, 11 \newline 12, 12 \newline 14, 13
    & 16, 17 \newline 9, 8 \newline 4, 6 \newline 4, 6
    & 16, 17\newline 5, 4 \newline 2, 4 \newline 4, 4 \\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 24
   & 24, 24\newline 24, 17  \newline 18, 19 \newline 15, 15
    & 24, 23 \newline 21, 10\newline 0, 0 \newline 0, 0
    & 24, 23 \newline 21, 9\newline 0, 0 \newline 0, 0\\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 23
     & 23, 23 \newline 21, 21 \newline 18, 18 \newline 18, 18
    & 23, 18 \newline 0, 5 \newline 0, 2 \newline 2, 3
    & 23, 18 \newline 0, 5 \newline 0, 2 \newline 2, 3\\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 18
    & 18, 18 \newline 12, 13  \newline 12, 12 \newline 13, 13
    & 17, 17 \newline 2, 8 \newline 3, 5 \newline 2, 7 
    & 17, 17 \newline 0, 6\newline 1, 3 \newline 2, 5\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 9
    & 9, 9 \newline 9, 9 \newline 9, 9 \newline 6, 6
    & 9, 9 \newline 3, 3 \newline 3, 3 \newline 2, 2
    & 9, 9 \newline 3, 3\newline 3, 3 \newline 2, 2  \\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 14
    & 14, 14 \newline 7, 7   \newline 6, 4 \newline 0, 6
    & 14, 14  \newline 3, 7 \newline 6, 7 \newline 1, 5
    & 14, 14 \newline 2, 5 \newline 4, 4 \newline 0, 1\\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 20
    & 20, 20  \newline 19, 19  \newline 15, 15 \newline 13, 15
    & 20, 20 \newline 8, 14 \newline 4, 6 \newline 2, 2
    & 20, 20 \newline 8, 14 \newline 3, 4 \newline 2, 2 \\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 33
    & 28, 28 \newline 21, 21  \newline 8, 8 \newline 11, 9  
    & 16, 10  \newline 3, 1 \newline 0, 2 \newline 0, 1
    & 16, 10 \newline 2, 1 \newline 0, 1 \newline 0, 1 \\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 24
   & 20, 18 \newline 11, 16 \newline 0, 3 \newline 6, 6
    & 24, 18 \newline 5, 12\newline 0, 11 \newline 0, 11
    & 20, 18 \newline 0, 11 \newline 0, 3 \newline 0, 2 \\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 17 \newline 11, 10  \newline 10, 12 \newline 10, 12 
    & 17, 17 \newline 3, 5 \newline 3, 4 \newline 1, 4
    & 17, 17 \newline 2, 3\newline 3, 3 \newline 1, 4 \\

\bottomrule
\end{tabular}
\label{tab:task1-gpt4omini}
\end{table*}



\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 2 results (gpt-4o-mini).}
\begin{tabular}{p{2.5cm}|p{4cm}|p{2.5cm}|p{4cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $C'$ \newline 
(judges: 0.6-sim, llama3.3-70b) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 15
     &14, 14 \newline 3, 6 \newline 1, 3 \newline 3, 5\\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 12
     &12, 12\newline 4, 6 \newline 5, 8 \newline 2, 1 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 19
     &15, 15 \newline 4, 6 \newline 4, 5 \newline 0, 2 \\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 17\newline 1, 7  \newline 1, 7 \newline 0, 1 \\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 22
    & 21, 21\newline 0, 4  \newline 0, 0 \newline 0, 0 \\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 20
    & 17, 17 \newline 7, 4 \newline 2, 3 \newline 1, 1 \\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 16
    & 16, 15 \newline 6, 5 \newline 5, 5 \newline 0, 1 \\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 12, 12\newline 4, 5 \newline 0, 0 \newline 0, 1 \\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 16, 16 \newline 2, 3 \newline 2, 2 \newline 3, 5 \\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 6
    & 6, 6 \newline 2, 3 \newline 2, 3 \newline 1, 1 \\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 9
    & 6, 5 \newline 4, 2\newline 4, 3 \newline 3, 4 \\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 12
    & 12, 12 \newline 1,  1 \newline 0, 0 \newline 0, 0 \\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 11
    & 9, 9 \newline 1, 3 \newline 0, 4 \newline 0, 0\\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 8
    & 3, 3\newline 0, 1 \newline 0, 0 \newline 0, 0 \\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 18, 18 \newline 2, 0 \newline 3, 2 \newline 1, 2 \\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    &16, 17 \newline 0, 2 \newline 1, 1 \newline 0, 0\\

\bottomrule
\end{tabular}
\label{tab:task2-gpt4omini}
\end{table*}



\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 3 results (gpt-4o-mini). }
\begin{tabular}{p{2.5cm}|p{4cm}|p{2.5cm}|p{4cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $S_i$ \newline 
(judges: 0.6-sim, llama3.3-70b ) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 13
     & 10, 8 \newline 4, 2 \newline 5, 3 \newline 5, 4 \\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 11
    &7, 7\newline 2, 2 \newline 2, 2 \newline 0, 0 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 14
     & 14, 9\newline 10, 6 \newline 10, 4 \newline 10, 5\\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 14, 8 \newline 7, 1 \newline 6, 2 \newline 3, 0\\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 28
    & 17, 15 \newline 0, 0 \newline 0, 0 \newline 0, 1 \\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 19, 16 \newline 11, 8\newline 6, 7 \newline 0, 0\\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 14
    & 7, 4 \newline 2, 1 \newline 2, 2 \newline 2, 1\\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 16, 13 \newline 5, 5 \newline 8, 7 \newline 2, 2\\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 6, 6 \newline 4, 4 \newline 9, 9 \newline 8, 8\\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 14 \newline 12, 13\newline 12, 13 \newline 7, 5\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 7
    & 7, 3\newline  4, 5\newline 4, 4 \newline 1, 1\\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 12
    & 12, 4 \newline 1, 1\newline 0, 0 \newline 1, 1\\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 10, 10\newline 8, 8\newline 2, 2 \newline 1, 2\\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 22
    & 11, 11 \newline 4, 4 \newline 6, 6 \newline 2, 2\\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 15, 13\newline 1, 2 \newline 1, 1 \newline 0, 0\\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 13, 12 \newline 1, 0 \newline 2, 0 \newline 3, 1\\

\bottomrule
\end{tabular}
\label{tab:task3-gpt4omini}
\end{table*}

==> eval-llama3.3-70b.tex <==

\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 1 results (llama3.3-70b).}
\begin{tabular}{p{2.2cm}|p{3.5cm}| p{1.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $s'$ \newline (judges: 0.6-sim, llama3.3-70b) &  \#Correct $A'$ \newline (judges: 0.6-sim, llama3.3-70b) & \#Correct both \newline (judges: 0.6-sim, llama3.3-70b) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 15
    & 15, 15 \newline 14, 14  \newline 14, 14 \newline 12, 13
    & 15, 13 \newline 5, 10 \newline 11, 10 \newline 11, 12 
    & 13, 13 \newline 4, 9 \newline 10, 9 \newline 9, 11 \\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 15
     & 15, 15 \newline 8, 8 \newline 8, 8 \newline 9, 10
    & 15, 15 \newline 0, 1 \newline 0, 1 \newline 0, 0
    & 15, 15 \newline 0, 1 \newline 0, 1 \newline 0, 0 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 27
     & 27, 27 \newline 25, 24 \newline 25, 25 \newline 24, 23 
    & 26, 27 \newline 17, 10 \newline 3, 8 \newline 7, 10 
    & 26, 27 \newline 15, 9 \newline 3, 8 \newline 7, 10 \\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted  \newline No context
    & 21
   & 21, 21 \newline 19, 18 \newline 18, 17 \newline 16, 12
    & 21, 21 \newline 8, 12 \newline 7, 8 \newline 3, 6
    & 21, 21 \newline 7, 10 \newline 6, 7 \newline 3, 5\\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 34
   & 34, 34\newline 19, 20 \newline 12, 14 \newline 9, 9
    & 34, 33 \newline 3, 10 \newline 3, 12 \newline 7, 10
    & 34, 33 \newline 2, 4 \newline 3, 4 \newline 0, 0\\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 21
    & 20, 20 \newline 16, 17 \newline 13, 16 \newline 3, 4
    & 20, 20 \newline 12, 10 \newline 6, 6 \newline 1, 4 
    & 20, 20 \newline 10, 9 \newline 6, 6 \newline 0, 0\\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 19, 19\newline 12, 11 \newline 12, 12 \newline 14, 13
    & 16, 17 \newline 9, 8 \newline 4, 6 \newline 4, 6
    & 16, 17\newline 5, 4 \newline 2, 4 \newline 4, 4 \\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 24
   & 24, 24\newline 24, 17  \newline 18, 19 \newline 15, 15
    & 24, 23 \newline 21, 10\newline 0, 0 \newline 0, 0
    & 24, 23 \newline 21, 9\newline 0, 0 \newline 0, 0\\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 23
     & 23, 23 \newline 21, 21 \newline 18, 18 \newline 18, 18
    & 23, 18 \newline 0, 5 \newline 0, 2 \newline 2, 3
    & 23, 18 \newline 0, 5 \newline 0, 2 \newline 2, 3\\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 18
    & 18, 18 \newline 12, 13  \newline 12, 12 \newline 13, 13
    & 17, 17 \newline 2, 8 \newline 3, 5 \newline 2, 7 
    & 17, 17 \newline 0, 6\newline 1, 3 \newline 2, 5\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 9
    & 9, 9 \newline 9, 9 \newline 9, 9 \newline 6, 6
    & 9, 9 \newline 3, 3 \newline 3, 3 \newline 2, 2
    & 9, 9 \newline 3, 3\newline 3, 3 \newline 2, 2  \\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 14
    & 14, 14 \newline 7, 7   \newline 6, 4 \newline 0, 6
    & 14, 14  \newline 3, 7 \newline 6, 7 \newline 1, 5
    & 14, 14 \newline 2, 5 \newline 4, 4 \newline 0, 1\\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 20
    & 20, 20  \newline 19, 19  \newline 15, 15 \newline 13, 15
    & 20, 20 \newline 8, 14 \newline 4, 6 \newline 2, 2
    & 20, 20 \newline 8, 14 \newline 3, 4 \newline 2, 2 \\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 33
    & 28, 28 \newline 21, 21  \newline 8, 8 \newline 11, 9  
    & 16, 10  \newline 3, 1 \newline 0, 2 \newline 0, 1
    & 16, 10 \newline 2, 1 \newline 0, 1 \newline 0, 1 \\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 24
   & 20, 18 \newline 11, 16 \newline 0, 3 \newline 6, 6
    & 24, 18 \newline 5, 12\newline 0, 11 \newline 0, 11
    & 20, 18 \newline 0, 11 \newline 0, 3 \newline 0, 2 \\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 17 \newline 11, 10  \newline 10, 12 \newline 10, 12 
    & 17, 17 \newline 3, 5 \newline 3, 4 \newline 1, 4
    & 17, 17 \newline 2, 3\newline 3, 3 \newline 1, 4 \\

\bottomrule
\end{tabular}
\label{tab:task1-llama}
\end{table*}



\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 2 results (llama3.3-70b).}
\begin{tabular}{p{2.5cm}|p{4cm}|p{2.5cm}|p{4cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $C'$ \newline 
(judges: 0.6-sim, llama3.3-70b) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 15
     &14, 14 \newline 3, 6 \newline 1, 3 \newline 3, 5\\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 12
     &12, 12\newline 4, 6 \newline 5, 8 \newline 2, 1 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 19
     &15, 15 \newline 4, 6 \newline 4, 5 \newline 0, 2 \\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 17\newline 1, 7  \newline 1, 7 \newline 0, 1 \\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 22
    & 21, 21\newline 0, 4  \newline 0, 0 \newline 0, 0 \\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 20
    & 17, 17 \newline 7, 4 \newline 2, 3 \newline 1, 1 \\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 16
    & 16, 15 \newline 6, 5 \newline 5, 5 \newline 0, 1 \\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 12, 12\newline 4, 5 \newline 0, 0 \newline 0, 1 \\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 16, 16 \newline 2, 3 \newline 2, 2 \newline 3, 5 \\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 6
    & 6, 6 \newline 2, 3 \newline 2, 3 \newline 1, 1 \\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 9
    & 6, 5 \newline 4, 2\newline 4, 3 \newline 3, 4 \\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 12
    & 12, 12 \newline 1,  1 \newline 0, 0 \newline 0, 0 \\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 11
    & 9, 9 \newline 1, 3 \newline 0, 4 \newline 0, 0\\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 8
    & 3, 3\newline 0, 1 \newline 0, 0 \newline 0, 0 \\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 18, 18 \newline 2, 0 \newline 3, 2 \newline 1, 2 \\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    &16, 17 \newline 0, 2 \newline 1, 1 \newline 0, 0\\

\bottomrule
\end{tabular}
\label{tab:task2-llama}
\end{table*}



\begin{table*}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.9}
\caption{Task 3 results (llama3.3-70b). }
\begin{tabular}{p{2.5cm}|p{4cm}|p{2.5cm}|p{4cm}}
\toprule
Protocol & Context type & \#Queries & \#Correct $S_i$ \newline 
(judges: 0.6-sim, llama3.3-70b ) \\
\midrule
TCP & Easy table \newline Manually-extracted rfc \newline  LLM-extracted \newline No context
    & 13
     & 10, 8 \newline 4, 2 \newline 5, 3 \newline 5, 4 \\
\midrule
TCP new reno & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 11
    &7, 7\newline 2, 2 \newline 2, 2 \newline 0, 0 \\
\midrule
SCTP & Easy table \newline Manually-extracted rfc  \newline LLM-extracted \newline No context
    & 14
     & 14, 9\newline 10, 6 \newline 10, 4 \newline 10, 5\\
\midrule
DCCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 14, 8 \newline 7, 1 \newline 6, 2 \newline 3, 0\\
\midrule
PPP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 28
    & 17, 15 \newline 0, 0 \newline 0, 0 \newline 0, 1 \\
\midrule
PPTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 19
    & 19, 16 \newline 11, 8\newline 6, 7 \newline 0, 0\\
\midrule
DHCP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 14
    & 7, 4 \newline 2, 1 \newline 2, 2 \newline 2, 1\\
\midrule
BGP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 16, 13 \newline 5, 5 \newline 8, 7 \newline 2, 2\\
\midrule
SMTP server & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 6, 6 \newline 4, 4 \newline 9, 9 \newline 8, 8\\
\midrule
POP3 & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 17, 14 \newline 12, 13\newline 12, 13 \newline 7, 5\\
\midrule
IMAP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 7
    & 7, 3\newline  4, 5\newline 4, 4 \newline 1, 1\\
\midrule
NNTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 12
    & 12, 4 \newline 1, 1\newline 0, 0 \newline 1, 1\\
\midrule
SIP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 15
    & 10, 10\newline 8, 8\newline 2, 2 \newline 1, 2\\
\midrule
RTSP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 22
    & 11, 11 \newline 4, 4 \newline 6, 6 \newline 2, 2\\
\midrule
FTP & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 15, 13\newline 1, 2 \newline 1, 1 \newline 0, 0\\
\midrule
MQTT & Easy table \newline Manually-extracted rfc \newline LLM-extracted \newline No context
    & 17
    & 13, 12 \newline 1, 0 \newline 2, 0 \newline 3, 1\\

\bottomrule
\end{tabular}
\label{tab:task3-llama}
\end{table*}

==> eval-temp.tex <==
\section*{Temperature effect}
Tables below show how the temperature selection affects the results of the experiment with llama3.3-70b.

\begin{table}[htbp]
\centering
\small
\label{tab:task1-metric-difficulty}
\caption{Metric difficulty on Task~1, 2, 3(smaller number is harder).}
\begin{tabular}{p{1cm}p{2cm}p{2cm}}
\toprule
Metric  & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0)
\\
\midrule
Both & 0.38 & 0.41 \\
$A'$ & 0.43 & 0.44 \\
$s'$ & 0.73 & 0.78 \\
$C'$ & 0.34 & 0.32 \\
$S_i$ & 0.36 & 0.38\\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[htbp]
\centering
\small
\caption{Overall performance on Task~1.}
\label{tab:task1-overall}
\begin{tabular}{p{2cm}p{2cm}p{2cm}}
\toprule
Judge  & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0) \\
\midrule
Overall  & 0.514 & 0.541   \\
Sim-0.6 & 0.49  &  0.52   \\
llama3.3-70b  & 0.53 & 0.57  \\

\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\small
\caption{Effect of context type on Task~1}
\label{tab:task1-context-effect}
\begin{tabular}
{p{2cm}p{2cm}p{2cm}}
\toprule
Context Type  & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0) \\
\midrule
Easy           & 0.94 &  0.95      \\
Manual-extraced-RFC  & 0.46& 0.50  \\
LLM-extracted-RFC   & 0.35 & 0.39  \\
No-context & 0.30  &  0.33   \\
\bottomrule
\end{tabular}
\end{table}





\begin{table}[htbp]
\centering
\small
\caption{Protocol-level difficulty on Task~1(smaller number is harder).}

\label{tab:task1-protocol-difficulty}
\begin{tabular}{p{2cm}p{2cm}p{2cm}}
\toprule
Protocol  & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0)  \\
\midrule
RTSP           &0.25& 0.30   \\
FTP            &0.37& 0.48  \\
TCP New Reno   &0.40&  0.41  \\
PPP            &0.42& 0.43  \\
NNTP           &0.47& 0.62  \\
SMTP Server    &0.48& 0.49  \\
MQTT           &0.50& 0.53  \\
PPTP           &0.51& 0.51  \\
POP3           &0.52& 0.55  \\
DHCP           &0.52& 0.51  \\
BGP            &0.54&  0.60 \\
SIP            &0.59& 0.59  \\
DCCP           &0.61& 0.61  \\
IMAP           &0.62& 0.62  \\
SCTP           &0.64&  0.66 \\
TCP            &0.77& 0.76  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[htbp]
\centering
\small
\caption{Overall performance on Task~2.}
\label{tab:task2-overall}
\begin{tabular}{p{2cm}p{2cm}p{2cm}}
\toprule
Judge & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0) \\
\midrule
Overall  & 0.342 & 0.321     \\
Sim-0.6 & 0.32  &  0.31      \\
llama3.3-70b  & 0.36 &  0.33 \\

\bottomrule
\end{tabular}
\end{table}

% \begin{table}[ht]
% \centering
% \small
% \caption{Metric difficulty on Task~2}
% \label{tab:task2-metric-difficulty}
% \begin{tabular}{lccc}
% \toprule
% Metric & 32B LLM 
% & llama3.3-70B 
% & GPT-4o-mini  \\
% \midrule
% $C'$ & 0.38 & 0.34 & 0.30 \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[htbp]
\centering
\small
\caption{Effect of context type on Task~2.}
\label{tab:task2-context-effect}
\begin{tabular}
{p{2cm}p{2.5cm}p{2cm}}
\toprule
Context Type  & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0) \\
\midrule
Easy          &0.87 & 0.87  \\
Manual-extracted-RFC  &0.22 & 0.19   \\
LLM-extracted-RFC  &0.18 &  0.15 \\
No-context  & 0.09& 0.07  \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\small
\caption{Protocol-level difficulty on Task~2 (smaller number is harder).}
\label{tab:task2-protocol-difficulty}
\begin{tabular}{p{2cm}p{2cm}p{2cm}}
\toprule
Protocol  & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0)  \\
\midrule
RTSP           & 0.11 & 0.09   \\
PPP            & 0.26 & 0.27  \\
MQTT           &0.27 & 0.27   \\
BGP            &0.28  & 0.28  \\
FTP            & 0.30 & 0.37  \\
NNTP           & 0.27 & 0.26  \\
SCTP            &0.34  & 0.26 \\
POP3           &0.50  & 0.50  \\
PPTP           &0.32  & 0.32  \\
SIP            &0.30 &  0.28   \\
TCP            &0.41 &  0.45   \\
DHCP           &0.41 & 0.41    \\
TCP New Reno  &0.52 &  0.32   \\
DCCP           &0.38 &  0.38  \\
SMTP Server    &0.36 & 0.30   \\
IMAP           &0.43 & 0.36   \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[htbp]
\centering
\small
\caption{Overall performance on Task~3.}
\label{tab:task3-overall}
\begin{tabular}{p{2cm}p{2cm}p{2cm}}
\toprule
Judge & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0) \\
\midrule
Overall  & 0.356 &0.376 \\
Sim-0.6  & 0.40 & 0.43  \\
llama3.3-70b  & 0.31 & 0.32 \\

\bottomrule
\end{tabular}
\end{table}

% \begin{table}[ht]
% \centering
% \small
% \caption{Metric difficulty on Task~3}
% \label{tab:task3-metric-difficulty}
% \begin{tabular}{lccc}
% \toprule
% Metric & 32B LLM & llama3.3-70B & GPT-4o-mini \\
% \midrule
% $S_i$ & 0.37 & 0.36 & 0.195 \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[htbp]
\centering
\small
\caption{Effect of context type on Task~3}
\label{tab:task3-context-effect}
\begin{tabular}
{p{2cm}p{2cm}p{2cm}}
\toprule
Context Type & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0)  \\
\midrule
Easy           &0.69 &  0.71           \\
Manual-extratced-RFC     &0.29 & 0.32 \\
LLM-extracted-RFC  &0.28 &  0.28      \\
No-context &0.16 &   0.20     \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\small
\caption{Protocol-level difficulty on Task~3(smaller number is harder).}
\label{tab:task3-protocol-difficulty}
\begin{tabular}{p{2cm}p{2cm}p{2cm}}
\toprule
Protocol & llama3.3-70B(temp=0.7) & llama3.3-70B(temp=0) \\
\midrule
DHCP            &0.15 & 0.21   \\
NNTP           & 0.21& 0.28   \\
TCP New Reno   & 0.25&  0.27  \\
MQTT           & 0.24&  0.26  \\
RTSP           & 0.26&  0.31  \\
FTP            & 0.24 & 0.35   \\
SIP            & 0.36 & 0.37  \\
PPP            & 0.15 & 0.17  \\
DCCP           & 0.34 &  0.31 \\
TCP            & 0.39 &  0.47  \\
SMTP Server    & 0.40 & 0.35  \\
SCTP           & 0.61 & 0.57   \\
BGP            & 0.43 & 0.44  \\
IMAP           & 0.52& 0.50   \\
PPTP           & 0.44 & 0.46  \\
POP3           & 0.68 & 0.70   \\
\bottomrule
\end{tabular}
\end{table}




==> problem.tex <==
\section{Problem definition}
We want to measure the LLM's understanding of network protocol logic, specifically we find that finite state machine is an important representation reflecting how a protocol executes. 

We define the ground truth of protocol logic to be either defined in the specification like RFC files or if that is not accessible but a reference implementation is available, then the reference implementation embeds the protocol logic. If none of the above exists, then we refer to such a scenario as no ground truth, and we may consider the code implementations that have a high probability of reflecting how the protocol works. 

\begin{enumerate}
    \item Specification exists: For the finite state machine, we either directly obtain it from the RFC files in textual or picture format, or extract it manually by reading the document and crafting a picture. We also manually extract the textual expression of such state machines from the picture, into a text file where each row includes ``Current State, Transition Conditions, Next State, Resulting Actions" and the whole file includes the number of transitions rows. 
    \item Reference implementation exists: We may believe that the traces or unit tests reflect the protocol behavior. Open-Source VS close-source. 

\end{enumerate}




To measure LLM's understanding, we design several question templates. With the input protocol ground truth information, we can fill the template questions into concrete questions against a specific protocol, as well as after we have LLM's answers, we use the ground truth information to compare based on a text similarity computation. 

One example question template looks like this:
\begin{promptbox}
I'll test your understanding of [protocol name] State Machine.
Assume your current state is [state name], and you satisfy the conditions [conditions name], can you predict which state you will transition to? Answer in the format <nextstate> nextstate </nextstate>.
Can you also predict if any resulting actions will happen, if there is nothing, answer NULL, otherwise, answer in the format <resulting\_action> action1, action2, ... </resulting\_action>.
\end{promptbox}

other possible question templates:
\begin{promptbox}
pair-wise:\\
Given the current state and a packet received, predict the next state and actions (the same we did before)
Given a state transition pair, ask it what condition caused that? (this might be multiple paths?)
Given a condition and next state, ask which previous state it was in? (this may also be multiple paths?)\\
\\
series-wise:
Given a series of packets, predict the current state the protocol party is in, and predict the next message (i.e. the result of a series of transitions)
Given a packet trace with a masked key field, ask it to predict that field? ( This is similar to figure out the intermediate state among a series of transitions )\\
\\
Critical-thinking:
Craft a trace which violates the state machine, ask it to detect if it's wrong and why?\\
\\
End-to-end understanding? 
Given a series of traces, ask it to construct the whole transition rules and the state machine? This is done by previous works? 

\end{promptbox}

==> tasks.tex <==
\section{Task Definition}
